Transductive Learning for Textual Few-Shot Classification in API-based Embedding Models

Proprietary and closed APIs are becoming increasingly common to process natural language, and are impacting the practical applications of natural language processing, including few-shot classification. Few-shot classification involves training a model to perform a new classification task with a handful of labeled data. This paper presents three contributions. First, we introduce a scenario where the embedding of a pre-trained model is served through a gated API with compute-cost and data-privacy constraints. Second, we propose a transductive inference, a learning paradigm that has been overlooked by the NLP community. Transductive inference, unlike traditional inductive learning, leverages the statistics of unlabeled data. We also introduce a new parameter-free transductive regularizer based on the Fisher-Rao loss, which can be used on top of the gated API embeddings. This method fully utilizes unlabeled data, does not share any label with the third-party API provider and could serve as a baseline for future research. Third, we propose an improved experimental setting and compile a benchmark of eight datasets involving multiclass classification in four different languages, with up to 151 classes. We evaluate our methods using eight backbone models, along with an episodic evaluation over 1,000 episodes, which demonstrate the superiority of transductive inference over the standard inductive setting.

==> tables/all_table.tex <==
\resizebox{\textwidth}{!}{\begin{tabular}{llrrrrrrrrrrrrrrrr}\toprule                 & {} & \multicolumn{16}{l}{accuracy} \\                 & task & \multicolumn{4}{l}{Banking} & \multicolumn{4}{l}{Clinic} & \multicolumn{4}{l}{Emotions} & \multicolumn{4}{l}{Tweet} \\                 & way & \multicolumn{2}{l}{10} & \multicolumn{2}{l}{5} & \multicolumn{2}{l}{10} & \multicolumn{2}{l}{5} & \multicolumn{2}{l}{10} & \multicolumn{2}{l}{5} & \multicolumn{2}{l}{10} & \multicolumn{2}{l}{5} \\                 & shot &        10 &         5 &        10 &         5 &        10 &         5 &        10 &         5 &        10 &         5 &        10 &         5 &        10 &         5 &        10 &         5 \\model & losses &           &           &           &           &           &           &           &           &           &           &           &           &           &           &           &           \\\midrule
all-MiniLM-L12-v2 & CE &  0.912813 &  0.888173 &  0.950960 &  0.935680 &  0.935480 &  0.910253 &  0.964773 &  0.946587 &  0.319227 &  0.265000 &  0.445467 &  0.392853 &  0.188000 &  0.168413 &  0.309067 &  0.285973 \\                 & FR &  0.932307 &  0.912720 &  0.964160 &  0.949867 &  0.970280 &  0.959093 &  0.985840 &  0.980640 &  0.332080 &  0.282387 &  0.461760 &  0.419733 &  0.187267 &  0.170227 &  0.306000 &  0.288347 \\                 & I &  0.914307 &  0.892120 &  0.954053 &  0.939040 &  0.957680 &  0.937040 &  0.980560 &  0.966747 &  0.327813 &  0.275587 &  0.454320 &  0.406373 &  0.190493 &  0.170933 &  0.312187 &  0.288107 \\                 & PT &  0.912053 &  0.886467 &  0.948320 &  0.931467 &  0.950707 &  0.917000 &  0.975280 &  0.949893 &  0.317907 &  0.260027 &  0.445013 &  0.389520 &  0.185907 &  0.165213 &  0.305653 &  0.284533 \\
all-mpnet-base-v2 & CE &  0.942920 &  0.920893 &  0.968373 &  0.953413 &  0.981600 &  0.973120 &  0.987387 &  0.982053 &  0.339347 &  0.283627 &  0.470027 &  0.421173 &  0.210547 &  0.187867 &  0.331680 &  0.305893 \\                 & FR &  0.959547 &  0.946880 &  0.978693 &       NaN &  0.991320 &  0.988667 &  0.995547 &  0.994373 &  0.344693 &  0.294320 &  0.493413 &  0.450480 &  0.208440 &  0.188027 &  0.335040 &  0.316987 \\                 & I &  0.950520 &  0.932400 &  0.974987 &  0.962453 &  0.988400 &  0.982547 &  0.994827 &  0.992080 &  0.349333 &  0.291213 &  0.486080 &  0.430720 &  0.214707 &  0.190893 &  0.341707 &  0.312027 \\                 & PT &  0.944253 &  0.922293 &  0.969413 &  0.954960 &  0.985987 &  0.978467 &  0.993173 &  0.988347 &  0.341160 &  0.281280 &  0.478507 &  0.422507 &  0.209493 &  0.185320 &  0.336453 &  0.309840 \\
distilroberta-base & CE &  0.618027 &  0.553427 &  0.699947 &  0.644213 &  0.941227 &  0.917040 &  0.965200 &  0.947787 &  0.220267 &  0.188853 &  0.341280 &  0.307707 &  0.234080 &  0.204067 &  0.366000 &  0.328667 \\                 & FR &  0.721227 &  0.636000 &  0.814693 &  0.729227 &  0.950973 &  0.930067 &  0.975600 &  0.962133 &  0.254613 &  0.205440 &  0.379387 &  0.316027 &  0.239960 &  0.203400 &  0.366880 &  0.324880 \\                 & I &  0.623467 &  0.552960 &  0.714773 &  0.651227 &  0.940280 &  0.915947 &  0.966907 &  0.950533 &  0.227680 &  0.193200 &  0.349947 &  0.311360 &  0.232533 &  0.202467 &  0.361547 &  0.328720 \\                 & PT &  0.585653 &  0.531680 &  0.670480 &  0.621973 &  0.937027 &  0.911400 &  0.962693 &  0.942907 &  0.210093 &  0.186173 &  0.327093 &  0.300747 &  0.222960 &  0.192507 &  0.351573 &  0.319147 \\
roberta-base & CE &  0.510960 &  0.454280 &  0.600747 &  0.552933 &  0.891467 &  0.850067 &  0.930453 &  0.892987 &  0.182120 &  0.161893 &  0.291307 &  0.267867 &  0.219573 &  0.191373 &  0.346080 &  0.313893 \\                 & FR &  0.650200 &  0.547347 &  0.747573 &  0.650773 &       NaN &  0.869467 &  0.949067 &  0.915760 &  0.222053 &  0.175773 &  0.338213 &  0.284800 &  0.228787 &  0.193840 &  0.352240 &  0.314373 \\                 & I &  0.518480 &  0.457613 &  0.610427 &  0.558160 &  0.890267 &  0.845360 &  0.932933 &  0.897520 &  0.188760 &  0.165493 &  0.301253 &  0.274053 &  0.218640 &  0.188347 &  0.342533 &  0.313360 \\                 & PT &  0.449453 &  0.415173 &  0.538747 &  0.508533 &  0.884093 &  0.839267 &  0.924987 &  0.887440 &  0.160987 &  0.151987 &  0.267093 &  0.256827 &  0.208107 &  0.179240 &  0.331093 &  0.303013 \\
roberta-large & CE &  0.253027 &  0.235387 &  0.351973 &  0.334453 &  0.789293 &  0.729253 &  0.858640 &  0.800213 &  0.117160 &  0.113187 &  0.226027 &  0.212853 &  0.136853 &  0.134200 &  0.235547 &  0.234160 \\                 & FR &  0.494773 &  0.368000 &  0.601440 &  0.472907 &  0.878547 &  0.809800 &  0.938427 &  0.883387 &  0.147427 &  0.128640 &  0.253573 &  0.228107 &  0.200413 &  0.171667 &  0.315467 &  0.287093 \\                 & I &  0.357360 &  0.302227 &  0.482853 &  0.428507 &  0.810373 &  0.746947 &  0.883787 &  0.830000 &  0.138667 &  0.126453 &  0.253733 &  0.230293 &  0.179893 &  0.161240 &  0.301973 &  0.274880 \\                 & PT &  0.206360 &  0.210267 &  0.317840 &  0.314400 &  0.778267 &  0.716400 &  0.849173 &  0.789440 &  0.113707 &  0.110347 &  0.223040 &  0.212053 &  0.132987 &  0.131187 &  0.231600 &  0.231680 \\
xlm-roberta-base & CE &       NaN &       NaN &  0.564213 &  0.526533 &  0.754400 &  0.714920 &  0.808267 &  0.762480 &  0.173507 &  0.156480 &  0.280133 &  0.258720 &  0.170507 &  0.155480 &  0.278080 &  0.263520 \\                 & FR &  0.679627 &  0.585813 &  0.771600 &  0.681173 &  0.854107 &  0.798880 &  0.904933 &  0.854507 &  0.228440 &  0.184240 &  0.355973 &  0.295067 &  0.204507 &  0.171533 &  0.321093 &  0.287360 \\                 & I &  0.545520 &  0.482560 &  0.642507 &  0.587013 &  0.783013 &  0.730213 &  0.840240 &  0.795333 &  0.197893 &  0.170160 &  0.319253 &  0.277093 &  0.184640 &  0.161813 &  0.300107 &  0.278907 \\                 & PT &  0.434987 &  0.393987 &  0.531360 &  0.495520 &  0.739093 &  0.698280 &  0.797680 &  0.751333 &  0.160333 &  0.148013 &  0.268267 &  0.248933 &  0.159067 &  0.146920 &  0.269387 &  0.255307 \\
xlm-roberta-base & CE &       NaN &       NaN &  0.564213 &  0.526533 &  0.754400 &  0.714920 &  0.808267 &  0.762480 &  0.173507 &  0.156480 &  0.280133 &  0.258720 &  0.170507 &  0.155480 &  0.278080 &  0.263520 \\                 & FR &  0.679627 &  0.585813 &  0.771600 &  0.681173 &  0.854107 &  0.798880 &  0.904933 &  0.854507 &  0.228440 &  0.184240 &  0.355973 &  0.295067 &  0.204507 &  0.171533 &  0.321093 &  0.287360 \\                 & I &  0.545520 &  0.482560 &  0.642507 &  0.587013 &  0.783013 &  0.730213 &  0.840240 &  0.795333 &  0.197893 &  0.170160 &  0.319253 &  0.277093 &  0.184640 &  0.161813 &  0.300107 &  0.278907 \\                 & PT &  0.434987 &  0.393987 &  0.531360 &  0.495520 &  0.739093 &  0.698280 &  0.797680 &  0.751333 &  0.160333 &  0.148013 &  0.268267 &  0.248933 &  0.159067 &  0.146920 &  0.269387 &  0.255307 \end{tabular}}

==> tables/overall_results.tex <==
\resizebox{\textwidth}{!}{\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr} \toprule task & \multicolumn{20}{l}{Tweet} & \multicolumn{20}{l}{Banking} & \multicolumn{20}{l}{Emotions} & \multicolumn{20}{l}{Clinic} \\ way & \multicolumn{5}{l}{5} & \multicolumn{5}{l}{10} & \multicolumn{5}{l}{5} & \multicolumn{5}{l}{10} & \multicolumn{5}{l}{5} & \multicolumn{5}{l}{10} & \multicolumn{5}{l}{5} & \multicolumn{5}{l}{10} & \multicolumn{5}{l}{5} & \multicolumn{5}{l}{10} & \multicolumn{5}{l}{5} & \multicolumn{5}{l}{10} & \multicolumn{5}{l}{5} & \multicolumn{5}{l}{10} & \multicolumn{5}{l}{5} & \multicolumn{5}{l}{10} \\ shot & \multicolumn{5}{l}{5} & \multicolumn{5}{l}{5} & \multicolumn{5}{l}{10} & \multicolumn{5}{l}{10} & \multicolumn{5}{l}{5} & \multicolumn{5}{l}{5} & \multicolumn{5}{l}{10} & \multicolumn{5}{l}{10} & \multicolumn{5}{l}{5} & \multicolumn{5}{l}{5} & \multicolumn{5}{l}{10} & \multicolumn{5}{l}{10} & \multicolumn{5}{l}{5} & \multicolumn{5}{l}{5} & \multicolumn{5}{l}{10} & \multicolumn{5}{l}{10} \\ losses &     CE &     PT &      H &      I &     FR &     CE &     PT &      H &      I &     FR &     CE &     PT &      H &      I &     FR &     CE &     PT &      H &      I &     FR &      CE &     PT &      H &      I &     FR &     CE &     PT &      H &      I &     FR &     CE &     PT &      H &      I &     FR &     CE &     PT &      H &      I &     FR &       CE &     PT &      H &      I &     FR &     CE &     PT &      H &      I &     FR &     CE &     PT &      H &      I &     FR &     CE &     PT &      H &      I &     FR &     CE &     PT &      H &      I &     FR &     CE &     PT &      H &      I &     FR &     CE &     PT &      H &      I &     FR &     CE &     PT &      H &      I &     FR \\ model                &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &         &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &          &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\ \midrule all-MiniLM-L12-v2    &  28.60 &  28.45 &  20.00 &  28.81 &  28.83 &  16.84 &  16.52 &  10.00 &  17.09 &  17.02 &  30.91 &  30.57 &  20.00 &  31.22 &  30.60 &  18.80 &  18.59 &  10.00 &  19.05 &  18.73 &   93.57 &  93.15 &  21.13 &  93.90 &  94.99 &  88.82 &  88.65 &  11.59 &  89.21 &  91.27 &  95.10 &  94.83 &  20.73 &  95.41 &  96.42 &  91.28 &  91.21 &  10.41 &  91.43 &  93.23 &    39.29 &  38.95 &  20.00 &  40.64 &  41.97 &  26.50 &  26.00 &  10.00 &  27.56 &  28.24 &  44.55 &  44.50 &  20.00 &  45.43 &  46.18 &  31.92 &  31.79 &  10.00 &  32.78 &  33.21 &  94.66 &  94.99 &  20.14 &  96.67 &  98.06 &  91.03 &  91.70 &  10.07 &  93.70 &  95.91 &  96.48 &  97.53 &  20.00 &  98.06 &  98.58 &  93.55 &  95.07 &  10.00 &  95.77 &  97.03 \\ all-distilroberta-v1 &  31.45 &  31.72 &  20.52 &  32.34 &  32.30 &  19.39 &  19.00 &  10.04 &  19.51 &  19.30 &  34.18 &  34.42 &  22.20 &  34.87 &  34.94 &  22.14 &  21.86 &  10.35 &  22.32 &  22.14 &   95.09 &  95.03 &  94.82 &  97.59 &  95.58 &  91.41 &  91.50 &  90.24 &  95.25 &  92.61 &  96.48 &  96.51 &  96.67 &  98.46 &  97.14 &  93.53 &  93.59 &  93.44 &  96.30 &  94.52 &    37.33 &  36.87 &  20.14 &  38.75 &  38.27 &  24.30 &  23.85 &  10.02 &  25.32 &  24.85 &  41.89 &  42.01 &  20.87 &  43.49 &  43.10 &  29.12 &  29.15 &  10.11 &  30.23 &  29.77 &  97.99 &  98.34 &  98.11 &  99.61 &  98.72 &  96.89 &  97.08 &  96.19 &  98.99 &  97.71 &  98.49 &  99.09 &  98.94 &  99.69 &  99.27 &  97.73 &  98.16 &  97.97 &  99.20 &  98.51 \\ all-mpnet-base-v2    &  30.59 &  30.98 &  20.00 &  31.20 &  31.70 &  18.79 &  18.53 &  10.00 &  19.09 &  18.80 &  33.17 &  33.65 &  20.00 &  34.17 &  33.50 &  21.05 &  20.95 &  10.00 &  21.47 &  20.84 &   95.34 &  95.50 &  39.28 &  96.25 &    NaN &  92.09 &  92.23 &  10.00 &  93.24 &  94.69 &  96.84 &  96.94 &  65.16 &  97.50 &  97.87 &  94.29 &  94.43 &  10.00 &  95.05 &  95.95 &    42.12 &  42.25 &  20.00 &  43.07 &  45.05 &  28.36 &  28.13 &  10.00 &  29.12 &  29.43 &  47.00 &  47.85 &  20.00 &  48.61 &  49.34 &  33.93 &  34.12 &  10.00 &  34.93 &  34.47 &  98.21 &  98.83 &  38.74 &  99.21 &  99.44 &  97.31 &  97.85 &  10.00 &  98.25 &  98.87 &  98.74 &  99.32 &  65.13 &  99.48 &  99.55 &  98.16 &  98.60 &  10.00 &  98.84 &  99.13 \\ distilroberta-base   &  32.87 &  31.91 &  20.00 &  32.87 &  32.49 &  20.41 &  19.25 &  10.00 &  20.25 &  20.34 &  36.60 &  35.16 &  20.00 &  36.15 &  36.69 &  23.41 &  22.30 &  10.00 &  23.25 &  24.00 &   64.42 &  62.20 &  20.00 &  65.12 &  72.92 &  55.34 &  53.17 &  10.00 &  55.30 &  63.60 &  69.99 &  67.05 &  20.00 &  71.48 &  81.47 &  61.80 &  58.57 &  10.00 &  62.35 &  72.12 &    30.77 &  30.07 &  20.00 &  31.14 &  31.60 &  18.89 &  18.62 &  10.00 &  19.32 &  20.54 &  34.13 &  32.71 &  20.00 &  34.99 &  37.94 &  22.03 &  21.01 &  10.00 &  22.77 &  25.46 &  94.78 &  94.29 &  20.00 &  95.05 &  96.21 &  91.70 &  91.14 &  10.70 &  91.59 &  93.01 &  96.52 &  96.27 &  20.00 &  96.69 &  97.56 &  94.12 &  93.70 &  10.00 &  94.03 &  95.10 \\ roberta-base         &  31.39 &  30.30 &  20.00 &  31.34 &  31.44 &  19.14 &  17.92 &  10.00 &  18.83 &  19.38 &  34.61 &  33.11 &  20.00 &  34.25 &  35.22 &  21.96 &  20.81 &  10.00 &  21.86 &  22.88 &   55.29 &  50.85 &  20.08 &  55.82 &  65.08 &  45.43 &  41.52 &  10.00 &  45.76 &  54.73 &  60.07 &  53.87 &  20.00 &  61.04 &  74.76 &  51.10 &  44.95 &  10.00 &  51.85 &  65.02 &    26.79 &  25.68 &  20.00 &  27.41 &  28.48 &  16.19 &  15.20 &  10.00 &  16.55 &  17.58 &  29.13 &  26.71 &  20.00 &  30.13 &  33.82 &  18.21 &  16.10 &  10.00 &  18.88 &  22.21 &  89.30 &  88.74 &  20.09 &  89.75 &  91.58 &  85.01 &  83.93 &  10.24 &  84.54 &  86.95 &  93.05 &  92.50 &  20.00 &  93.29 &  94.91 &  89.15 &  88.41 &  10.00 &  89.03 &    NaN \\ roberta-large        &  23.42 &  23.17 &  20.41 &  27.49 &  28.71 &  13.42 &  13.12 &  10.29 &  16.12 &  17.17 &  23.55 &  23.16 &  20.72 &  30.20 &  31.55 &  13.69 &  13.30 &  10.44 &  17.99 &  20.04 &   33.45 &  31.44 &  26.93 &  42.85 &  47.29 &  23.54 &  21.03 &  13.64 &  30.22 &  36.80 &  35.20 &  31.78 &  27.77 &  48.29 &  60.14 &  25.30 &  20.64 &  14.25 &  35.74 &  49.48 &    21.29 &  21.21 &  20.96 &  23.03 &  22.81 &  11.32 &  11.03 &  10.62 &  12.65 &  12.86 &  22.60 &  22.30 &  21.81 &  25.37 &  25.36 &  11.72 &  11.37 &  11.02 &  13.87 &  14.74 &  80.02 &  78.94 &  20.00 &  83.00 &  88.34 &  72.93 &  71.64 &  10.00 &  74.69 &  80.98 &  85.86 &  84.92 &  20.00 &  88.38 &  93.84 &  78.93 &  77.83 &  10.00 &  81.04 &  87.85 \\ xlm-roberta-base     &  26.35 &  25.53 &  20.12 &  27.89 &  28.74 &  15.55 &  14.69 &  10.01 &  16.18 &  17.15 &  27.81 &  26.94 &  20.07 &  30.01 &  32.11 &  17.05 &  15.91 &  10.01 &  18.46 &  20.45 &   52.65 &  49.55 &  20.50 &  58.70 &  68.12 &    NaN &  39.40 &  10.19 &  48.26 &  58.58 &  56.42 &  53.14 &  20.44 &  64.25 &  77.16 &    NaN &  43.50 &  10.07 &  54.55 &  67.96 &    25.87 &  24.89 &  20.39 &  27.71 &  29.51 &  15.65 &  14.80 &  10.06 &  17.02 &  18.42 &  28.01 &  26.83 &  20.37 &  31.93 &  35.60 &  17.35 &  16.03 &  10.10 &  19.79 &  22.84 &  76.25 &  75.13 &  20.31 &  79.53 &  85.45 &  71.49 &  69.83 &  10.63 &  73.02 &  79.89 &  80.83 &  79.77 &  20.30 &  84.02 &  90.49 &  75.44 &  73.91 &  10.09 &  78.30 &  85.41 \\ xlm-roberta-large    &  24.84 &  24.45 &  20.21 &  26.65 &  26.57 &  13.82 &  13.46 &  10.08 &  14.89 &  15.12 &  25.87 &  25.42 &  20.33 &  28.31 &  28.80 &  14.91 &  14.59 &  10.10 &  16.88 &  17.78 &   41.37 &  39.62 &  21.26 &  49.34 &  55.99 &  31.36 &  28.45 &  10.24 &  37.06 &  44.94 &  45.08 &  42.93 &  22.04 &  55.58 &  67.29 &  35.13 &  31.63 &  10.26 &  43.79 &  56.64 &    22.15 &  21.99 &  20.15 &  22.93 &  23.11 &  12.04 &  11.87 &  10.01 &  12.59 &  12.88 &  22.85 &  22.80 &  20.15 &  24.70 &  25.26 &  12.71 &  12.33 &  10.02 &  13.75 &  14.41 &  60.54 &  59.49 &  20.36 &  67.37 &  75.10 &  52.18 &  50.83 &  10.11 &  57.60 &  66.43 &  65.97 &  65.25 &  20.63 &  74.45 &  83.83 &  56.56 &  55.34 &  10.11 &  64.01 &  75.60 \\ xlm-roberta-xl       &  30.53 &  30.28 &  20.00 &  30.76 &  30.66 &  18.06 &  17.78 &  10.00 &  18.17 &  18.17 &  33.32 &  32.81 &  20.00 &  33.33 &  33.44 &  20.61 &  20.26 &  10.00 &  20.74 &  20.89 &   84.29 &  83.19 &  20.91 &  84.17 &  84.60 &  76.46 &  75.07 &  14.42 &  74.03 &  76.37 &  89.16 &  88.86 &  20.04 &  89.35 &  89.53 &  83.07 &  82.57 &  10.40 &  82.27 &  83.24 &    35.78 &  35.05 &  20.00 &  36.10 &  35.93 &  23.22 &  22.61 &  10.00 &  23.04 &  23.43 &  41.35 &  41.13 &  20.00 &  41.91 &  42.43 &  28.11 &  27.47 &  10.00 &  28.17 &  28.47 &  93.06 &  91.98 &  24.70 &  92.62 &  93.47 &  89.55 &  88.15 &  22.49 &  87.20 &  89.50 &  95.45 &  95.09 &  21.61 &  95.46 &  95.79 &  92.84 &  92.27 &  13.43 &  91.95 &  93.00 \\ \bottomrule \end{tabular}}

==> tables/total.tex <==
\begin{table}
    \centering
 \begin{tabular}{lrrrr} \hline
 way &     10 &      5 &     10 &      5 \\
 shot &     10 &     10 &      5 &      5 \\ 
 losses &        &        &        &        \\ 
 CE     &  50.30 &  58.74 &  47.19 &  55.79 \\ FR     &  55.22 &  65.79 &  51.72 &  60.61 \\ H      &  17.87 &  29.62 &  17.67 &  28.00 \\ I      &  52.37 &  61.18 &  48.63 &  57.72 \\ PT     &  49.34 &  57.99 &  46.32 &  55.15 \\ 


 \end{tabular}\caption{Caption}\label{tab:my_label}
\end{table}

